Leveraging Multimodal Fusion for Enhanced Diagnosis of Multiple Retinal Diseases in Ultra-wide OCTA

Ultra-wide optical coherence tomography angiography (UW-OCTA) is an emerging imaging technique that offers significant advantages over traditional OCTA by providing an exceptionally wide scanning range of up to 24 x 20 $mm^{2}$, covering both the anterior and posterior regions of the retina. However, the currently accessible UW-OCTA datasets suffer from limited comprehensive hierarchical information and corresponding disease annotations. To address this limitation, we have curated the pioneering M3OCTA dataset, which is the first multimodal (i.e., multilayer), multi-disease, and widest field-of-view UW-OCTA dataset. Furthermore, the effective utilization of multi-layer ultra-wide ocular vasculature information from UW-OCTA remains underdeveloped. To tackle this challenge, we propose the first cross-modal fusion framework that leverages multi-modal information for diagnosing multiple diseases. Through extensive experiments conducted on our openly available M3OCTA dataset, we demonstrate the effectiveness and superior performance of our method, both in fixed and varying modalities settings. The construction of the M3OCTA dataset, the first multimodal OCTA dataset encompassing multiple diseases, aims to advance research in the ophthalmic image analysis community.

==> discussion.tex <==
\section{discussion}
Through extensive experiments, the effectiveness and stability of the proposed fusion method have been proved. Within an identical field of view, the acquisition of a greater volume of information is advantageous for diagnosis, irrespective of whether this information is redundant or exhibits varying specificities. However, our experiment should be augmented by cropping an area equivalent to the FOV of conventional OCTA. Which will allow us to quantitatively ascertain that the ultra-wide range possesses superior diagnostic efficacy compared to traditional OCTA. Furthermore, examining the influence of the different resolutions of the input image on the diagnostic outcome undeniably constitutes a more clinically pertinent methodology. Beyond the fusion method, we delved deeper into the potential application of retina-related foundational models on Ultra-Widefield Optical Coherence Tomography Angiography (UW-OCTA). Our findings suggest that to fully harness the potential of artificial intelligence within the field of ophthalmology, it is essential to incorporate novel information derived from innovative modalities with established foundational models.
